Specification-Driven Code Translation Powered by Large Language Models: How Far Are We?

Large Language Models (LLMs) are increasingly being applied across various domains, including code-related tasks such as code translation. Previous studies have explored using LLMs for translating code between different programming languages. Since LLMs are more effective with natural language, using natural language as an intermediate representation in code translation tasks is an intuitively appealing approach. However, whether this benefit is general or highly context-dependent remains unclear. In this work, we investigate using NL-specification as an intermediate representation for code translation. We evaluate our method using three datasets, five popular programming languages, and 29 language pair permutations. Our results show that using NL-specification alone does not lead to performance improvements. However, when combined with source code, it provides gains in certain language pairs (notably with Python and C++ as source languages), while offering no consistent improvement overall. Besides analyzing the performance of code translation, we also investigate the quality of the translated code and provide insights into the issues present in the translated code.

==> disscussion.tex <==
{\color{blue}
\section{Prescriptive Recommendations for Practitioners}
Based on our empirical findings across multiple datasets and language pairs, we offer the following practical recommendations for practitioners applying LLM-based code translation in real-world settings:
\begin{itemize}
    \item \textbf{Prefer source-only translation as a strong baseline.} Across most language pairs, source-only translation achieves high computational accuracy and remains a reliable default. Practitioners should first evaluate source-only translation before introducing additional complexity.
    \item \textbf{Use \specS as a complementary strategy, not a replacement.} \specS and \specS combined with source code do not consistently outperform source-only translation. However, they often solve a small but distinct subset of problems that source-only translation fails. Practitioners may benefit from selectively applying \specS to difficult or failure-prone cases rather than using it uniformly.
    \item \textbf{Expect language-pair–specific behavior.} The effectiveness of \specS varies substantially across source–target language pairs. Practitioners should validate translation strategies on representative samples of their target language pairs rather than assuming uniform gains.
    \item \textbf{Ensure consistent and well-defined test suites.} Reliable evaluation depends critically on executable and unambiguous test cases. Practitioners should audit and repair test suites before comparing translation strategies, and apply identical evaluation protocols across all methods to avoid biased conclusions.
\end{itemize}
}

==> intertrans_comp.tex <==
\begin{table}
\color{blue}
\centering
\tiny
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.2}
\caption{\color{blue}Comparative analysis of translation performance on CodeNet using MagiCoder with and without Rust and JavaScript as target Languages, compared to the Intertrans \citep{macedo2024intertrans}}
\begin{tabular}{|
p{1.3cm}|
p{1.2cm}p{1.2cm}|
p{1.2cm}p{1.2cm}|
p{1.2cm}p{1.2cm}|
p{1.2cm}p{1.2cm}|}
\hline
\textbf{} &
\multicolumn{2}{p{2.4cm}|}{\centering\textbf{With Only \specS}} &
\multicolumn{2}{p{2.4cm}|}{\centering\textbf{With Only Source}} &
\multicolumn{2}{p{2.4cm}|}{\centering\textbf{With \specS + Source}} &
\multicolumn{2}{p{2.4cm}|}{\centering\textbf{InterTrans}} \\
\cline{2-9}
\textbf{Source Language} &
\textbf{All Target Langs.} & \textbf{Without Rust and JS} &
\textbf{All Target Langs.} & \textbf{Without Rust and JS} &
\textbf{All Target Langs.} & \textbf{Without Rust and JS} &
\textbf{All Target Langs.} & \textbf{Without Rust and JS} \\
\hline
Python     & 32.57 & 49.52 & 54.29 & 75.24 & 52.57 & 76.19 & 91.43 & 93.34 \\
Java       & 30.29 & 41.90 & 55.43 & 73.33 & 49.14 & 67.62 & 85.14 & 91.43 \\
C++        & 34.29 & 51.43 & 57.71 & 82.86 & 54.29 & 80.00 & 88.00 & 94.29 \\
Go         & 42.86 & 50.48 & 59.29 & 74.29 & 69.29 & 80.95 & 85.71 & 90.48 \\
Javascript & 28.00 & 32.38 & 55.43 & 62.86 & 57.71 & 65.71 & 87.43 & 87.86 \\
Rust       & 37.14 & 40.95 & 69.29 & 70.48 & 67.14 & 71.43 & 86.29 & 88.57 \\
\hline
\end{tabular}
\label{tab:js_rust_issue}
\end{table}

==> magicoder_it_res.tex <==
\begin{table*}
\color{blue}
\centering
\scriptsize
\renewcommand{\arraystretch}{1.1} % Improve row spacing
\caption{\color{blue}Code translation results after fixing errors using MagiCoder, compared to the Intertrans \citep{macedo2024intertrans}). Values in parentheses with ($\uparrow$) indicate the absolute improvement in correctness after error fixing, compared to the original translation results without fixing.}
\resizebox{\textwidth}{!}{  
\begin{tabular}{|m{1.6cm}|m{1.2cm}|m{2cm}|m{1cm}|m{1.1 cm}|m{1.4cm}|m{1.85cm}|m{1.85cm}|}
\hline
\textbf{Dataset} & \textbf{Source Language} & \textbf{Target Language(s)} & \textbf{Total Datapoints} & \textbf{Inter trans} & \textbf{With Only Source} & \textbf{With Only \specS} & \textbf{With \specS+ Source} \\
\hline
% \multirow{2}{*}{Avatar} & Python & C, C++, Go, Java & 956 & - & 53.33\% (15.83\%$\uparrow$) & 32.08\% (5.0\%$\uparrow$) & 57.5\% (6.25\%$\uparrow$)\\
% \cline{2-3} \cline{5-8}
% & Java & C, C++, Go, Python & 960 & - & 61.25\% (2.92\%$\uparrow$) & 21.25\% (2.92\%$\uparrow$) & 57.5\% (0.42\%$\uparrow$)\\
% \hline

% \multirow{5}{*}{Codenet} & C & C++, Go, Java, Python & \multirow{6}{*}{4000} & - & 81.38\% (6.13\%$\uparrow$) & 44.88\% (7.88\%$\uparrow$) & 80.5\% (6.12\%$\uparrow$)\\
% \cline{2-3} \cline{5-8}
% & C++ & C, Go, Java, Python &  & - & 80.12\% (8.74\%$\uparrow$) & 55.0\% (7.75\%$\uparrow$) & 81.25\% (5.87\%$\uparrow$)\\
% \cline{2-3} \cline{5-8}
% & Go & C, C++, Java, Python &  & - & 74.5\% (4.0\%$\uparrow$) & 53.75\% (5.5\%$\uparrow$) & 77.25\% (4.13\%$\uparrow$)\\
% \cline{2-3} \cline{5-8}
% & Java & C, C++, Go, Python &  & - &  75.75\% (8.5\%$\uparrow$) & 43.0\% (6.12\%$\uparrow$) & 74.5\% (7.12\%$\uparrow$)\\
% \cline{2-3} \cline{5-8}
% & Python & C, C++, Go, Java &  & - & 79.88\% (9.26\%$\uparrow$) & 62.0\% (5.88\%$\uparrow$) & 80.0\% (7.25\%$\uparrow$)\\
% \hline

\multirow{6}{*}{\parbox{1.3cm}{\centering CodeNet\\(InterTrans)}} & C++ & Go, Java, Python, JavaScript, Rust & \multirow{6}{*}{1050} & 88.0\% & 57.71\% (10.28\%$\uparrow$) & 34.29\% (5.15\%$\uparrow$) & 54.29\% (8.0\%$\uparrow$)\\
\cline{2-3} \cline{5-8}
 & Go & C++, Java, Python, JavaScript, Rust &  & 85.7\% & 59.29\% (8.58\%$\uparrow$) & 42.86\% (7.15\%$\uparrow$) & 69.29\% (12.86\%$\uparrow$)\\
 \cline{2-3} \cline{5-8}
 & Java & C++, Go, Python, JavaScript, Rust &  & 85.1\% & 55.43\% (18.86\%$\uparrow$) & 30.29\% (9.15\%$\uparrow$) & 49.14\% (13.71\%$\uparrow$)\\
 \cline{2-3} \cline{5-8}
 & Python & C++, Go, Java, JavaScript, Rust &  & 91.4\% & 54.29\% (18.29\%$\uparrow$) & 32.57\% (6.28\%$\uparrow$) & 52.57\% (15.43\%$\uparrow$)\\
 \cline{2-3} \cline{5-8}
 & JavaScript & C++, Go, Java, Python, Rust &  & 87.4\% & 55.43\% (39.28\%$\uparrow$) & 29.29\% (23.58\%$\uparrow$) & 58.57\% (44.28\%$\uparrow$)\\
 \cline{2-3} \cline{5-8}
 & Rust & C++, Go, Java, Python, JavaScript &  & 86.3\% & 70.48\% (4.77\%$\uparrow$) & 40.95\% (5.71\%$\uparrow$) & 71.43\% (6.67\%$\uparrow$)\\
\hline
% Evalplus & Python & Java & 164 & - &  84.15\% (41.47\%$\uparrow$) & 99.39\% (27.44\%$\uparrow$) & 93.9\% (32.92\%$\uparrow$) \\
% \hline
\end{tabular}
}
\label{tab:magicoder_it_results}
\end{table*}


==> main_result.tex <==
% \begin{table*}[]
% \color{red}
% \centering
% \tiny
% \setlength{\tabcolsep}{4pt}
% % \begin{tabular}{|l|l|c|c|c|c|c|c|c|c|c|}
% \begin{tabular}{|p{1.2cm}|p{1.1cm}|c|c|c|c|c|c|c|c|c|}
% \hline
% \textbf{Dataset} & \textbf{Src} &
% \multicolumn{3}{c|}{\textbf{GPT-4}} &
% \multicolumn{3}{c|}{\textbf{Magicoder}} &
% \multicolumn{3}{c|}{\textbf{DeepSeek}} \\
% \cline{3-11}
%  & &
%  N & S & N+S &
%  N & S & N+S &
%  N & S & N+S \\
% \hline

% Avatar & Python & 61.51 & 56.9 & 65.17 & 32.08 & 53.33 & 57.50 & 98.33 & 97.92 & 98.75 \\
%  & Java & 73.13 & 78.75 & 83.85 & 21.25 & 61.25 & 57.50 & 92.50 & 97.08 & 96.25 \\
% \hline
% Codenet & Python & 83.13 & 83.63 & 89.5 & 62.00 & 79.88 & 80.00 & 97.50 & 98.50 & 98.75 \\
%  & Java & 76.38 & 84.38 & 83.25 & 43.00 & 75.75 & 74.50 & 93.88 & 96.12 & 95.00 \\
%  & C & 70.75 & 88.63 & 84.63 & 44.88 & 81.38 & 80.50 & 95.62 & 97.12 & 97.00 \\
%  & C++ & 77.5 & 84.63 & 87.63 & 55.00 & 80.12 & 81.25 & 95.25 & 98.62 & 97.00 \\
%  & Go & 77.63 & 91.13 & 86.13 & 53.75 & 74.50 & 77.25 & 94.50 & 97.25 & 96.38 \\
% \hline
% Codenet & C++ & - & - & - & 33.14 & 49.71 & 49.71 & 82.29 & 92.00 & 89.71 \\
% (Intertrans) & Java & - & - & - & 26.29 & 48.00 & 42.29 & 84.57 & 87.43 & 88.00 \\
%  & Python & - & - & - & 30.29 & 46.86 & 47.43 & 88.57 & 96.00 & 94.86 \\
%  & Rust & - & - & - & 29.71 & 55.43 & 53.71 & 86.29 & 91.43 & 90.29 \\
%  & Go & - & - & - & 32.00 & 48.00 & 50.29 & 85.14 & 89.14 & 87.43 \\
%  & Javascript & - & - & - & - & - & - & 82.86 & 92.57 & 94.29 \\
% \hline
% Evalplus & Python & 79.27 & 84.76 & 85.37 & 99.39 & 84.15 & 93.90 & 82.32 & 81.10 & 82.93 \\
% \hline
% \end{tabular}
% \caption{(will update with src|nl|src+nl|intertrans) Code translation results across datasets, models. N: NL, S: Source, N+S: NL+Source.}
% \label{tab:code_translation_results}
% \end{table*}


==> main_results_with_intertrans.tex <==
\begin{table*}
\color{red}
\centering
\tiny
\setlength{\tabcolsep}{4pt}
% \begin{tabular}{|l|l|c|c|c|c|c|c|c|c|c|}
\begin{tabular}{|p{1.2cm}|p{1.1cm}|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Dataset} & \textbf{Src} &
\multicolumn{4}{c|}{\textbf{GPT-4}} &
\multicolumn{4}{c|}{\textbf{Magicoder}} &
\multicolumn{4}{c|}{\textbf{DeepSeek}} \\
\cline{3-14}
 & &
 N & S & N+S & IT &
 N & S & N+S & IT &
 N & S & N+S & IT \\
\hline

Avatar & Python & 61.51 & 56.9 & 65.17 & - & 32.08 & 53.33 & 57.50 & - & 98.33 & 97.92 & 98.75 & - \\
 & Java & 73.13 & 78.75 & 83.85 & - & 21.25 & 61.25 & 57.50 & - & 92.50 & 97.08 & 96.25 & - \\
\hline
Codenet & C++ & 77.5 & 84.63 & 87.63 & - & 55.00 & 80.12 & 81.25 & - & 95.25 & 98.62 & 97.00 & - \\
 & Go & 77.63 & 91.13 & 86.13 & - & 53.75 & 74.50 & 77.25 & - & 94.50 & 97.25 & 96.38 & - \\
 & Java & 76.38 & 84.38 & 83.25 & - & 43.00 & 75.75 & 74.50 & - & 93.88 & 96.12 & 95.00 & - \\
 & Python & 83.13 & 83.63 & 89.5 & - & 62.00 & 79.88 & 80.00 & - & 97.50 & 98.50 & 98.75 & - \\
 & C & 70.75 & 88.63 & 84.63 & - & 44.88 & 81.38 & 80.50 & - & 95.62 & 97.12 & 97.00 & - \\
\hline
Codenet & C++ & - & - & - & - & 34.29 & 57.71 & 54.29 & 88.0 & 82.29 & 92.00 & 89.71 & - \\
 (Intertrans) & Go & - & - & - & - & 42.86 & 59.29 & 69.29 & 85.7 & 85.14 & 89.14 & 87.43 & - \\
 & Java & - & - & - & - & 30.29 & 55.43 & 49.14 & 85.1 & 84.57 & 87.43 & 88.00 & - \\
 & Javascript & - & - & - & - & 28.00 & 55.43 & 57.71 & 87.4 & 82.86 & 92.57 & 94.29 & - \\
 & Python & - & - & - & - & 32.57 & 54.29 & 52.57 & 91.4 & 88.57 & 96.00 & 94.86 & - \\
 & Rust & - & - & - & - & 37.14 & 69.29 & 67.14 & 86.3 & 86.29 & 91.43 & 90.29 & - \\
\hline
Evalplus & Python & 79.27 & 84.76 & 85.37 & - & 99.39 & 84.15 & 93.90 & - & 82.32 & 81.10 & 82.93 & - \\
\hline
\end{tabular}
\caption{Code translation results across datasets, models. N: NL, S: Source, N+S: NL+Source, IT: Intertrans~\citep{macedo2024intertrans}.}
\label{tab:code_translation_results}
\end{table*}


==> significance_test_results.tex <==
\begin{table*}
\color{blue}
\centering
\scriptsize
\renewcommand{\arraystretch}{1.1}
\caption{\color{blue}
Paired significance and complementarity analysis across datasets and language pairs on DeepSeekCoder result. SC = source-only translation, NL = translation using \specS, SL = source language, TL = target languages. Fixes ($c$) = problems solved by the second method but not by the first, regressions ($b$) = problems solved by the first method but not by the second. $p$-values are computed using McNemar’s exact test on paired per-problem outcomes ($\alpha$ = 0.05).\fazle{highline p<0.05}
}
\resizebox{\textwidth}{!}{  
\begin{tabular}{|m{1.4cm}|m{1.8cm}|m{1.2cm}|m{1.6cm}|m{1.2cm}|m{1.2cm}|m{1.4cm}|m{1.4cm}|}
\hline
\textbf{Dataset} & \textbf{SL$\rightarrow$TL} & \textbf{Total} & \textbf{Only Source Correct (\%)} & \textbf{p (SC vs NL)} & \textbf{c/b (SC vs NL)} & \textbf{p (SC vs NL+SC)} & \textbf{c/b (SC vs NL+SC)} \\
\hline

\multirow{8}{*}{Avatar}
 & Java$\rightarrow$C        & 240 & 96.7  & 0.049  & 4/13 & 0.0625 & 5/0  \\
 & Java$\rightarrow$C++      & 240 & 98.8  & 1      & 1/2  & 1      & 1/2  \\
 & Java$\rightarrow$Go       & 240 & 92.9  & 0.824  & 11/9 & 0.0923 & 10/3 \\
 & Java$\rightarrow$Python   & 240 & 97.1  & 0.0266 & 5/16 & 0.754  & 4/6  \\
 & Python$\rightarrow$C      & 239 & 89.5  & 0.815  & 8/10 & 0.824  & 11/9 \\
 & Python$\rightarrow$C++    & 239 & 95.8  & 0.227  & 3/8  & 0.375  & 1/4  \\
 & Python$\rightarrow$Go     & 239 & 88.3  & 0.0989 & 13/24& 0.856  & 16/14\\
 & Python$\rightarrow$Java   & 239 & 97.9  & 1      & 4/3  & 0.688  & 4/2  \\
\hline

\multirow{16}{*}{CodeNet}
 & C$\rightarrow$C++         & 200 & 97.5  & 0.625  & 3/1  & 0.125  & 4/0  \\
 & C$\rightarrow$Go          & 200 & 95.5  & 0.508  & 6/3  & 0.0312 & 6/0  \\
 & C$\rightarrow$Java        & 200 & 98.5  & 0.0391 & 1/8  & 1      & 2/1  \\
 & C$\rightarrow$Python      & 200 & 97.0  & 0.0129 & 2/12 & 0.00183& 1/13 \\
 & C++$\rightarrow$C         & 200 & 99.5  & 0.219  & 1/5  & 0.219  & 1/5  \\
 & C++$\rightarrow$Go        & 200 & 100   & 0.0312 & 0/6  & 0.25   & 0/3  \\
 & C++$\rightarrow$Java      & 200 & 99.5  & 0.0703 & 1/7  & 1      & 1/0  \\
 & C++$\rightarrow$Python    & 200 & 95.5  & 0.0266 & 5/16 & 0.118  & 4/11 \\
 & Go$\rightarrow$C          & 200 & 96.5  & 0.227  & 3/8  & 1      & 5/4  \\
 & Go$\rightarrow$C++        & 200 & 98.5  & 0.289  & 2/6  & 1      & 2/3  \\
 & Go$\rightarrow$Java       & 200 & 100   & 0.0625 & 0/5  & 0.25   & 0/3  \\
 & Go$\rightarrow$Python     & 200 & 94.0  & 0.0768 & 4/12 & 0.454  & 6/10 \\
 & Java$\rightarrow$C        & 200 & 97.5  & 1      & 4/4  & 0.625  & 3/1  \\
 & Java$\rightarrow$C++      & 200 & 98.0  & 0.0625 & 0/5  & 0.625  & 1/3  \\
 & Java$\rightarrow$Go       & 200 & 93.5  & 1      & 6/6  & 1      & 6/6  \\
 & Java$\rightarrow$Python   & 200 & 95.5  & 0.00443& 3/16 & 0.0225 & 2/11 \\
 & Python$\rightarrow$C      & 200 & 98.0  & 1      & 3/3  & 1      & 2/1  \\
 & Python$\rightarrow$C++    & 200 & 99.5  & 0.5    & 0/2  & 1      & 0/0  \\
 & Python$\rightarrow$Go     & 200 & 97.5  & 0.109  & 2/8  & 1      & 1/1  \\
 & Python$\rightarrow$Java   & 200 & 99.0  & 1      & 1/1  & 1      & 1/0  \\
\hline

EvalPlus
 & Python$\rightarrow$Java   & 164 & 81.1  & 0.727  & 5/3  & 0.453  & 5/2  \\
\hline
\end{tabular}
}
\label{tab:significance_result}
\end{table*}


==> significance_test_results_union.tex <==
\begin{table*}

\centering
\scriptsize
\renewcommand{\arraystretch}{1.1}
\caption{
Paired significance and complementarity analysis across datasets and language pairs on DeepSeekCoder result. SC = source-only translation, NL = translation using \\specS, SL = source language, TL = target languages. Fixes ($c$) = problems solved by the second method but not by the first, regressions ($b$) = problems solved by the first method but not by the second. $p$-values are computed using McNemar’s exact test on paired per-problem outcomes ($\alpha$ = 0.05). Union comparisons quantify the combining effect using McNemar’s exact test between SC and an OR-ensemble of the other strategies. Cells shaded in green indicate statistically significant improvements over SC ($p<0.05$ and $c>b$), while red indicates statistically significant degradations ($p<0.05$ and $c<b$).
}
\resizebox{\textwidth}{!}{
\begin{tabular}{|m{1.2cm}|m{1.8cm}|m{0.8cm}|m{1.1cm}|m{0.6cm}|m{1.2cm}|m{0.6cm}|m{1.8cm}|m{0.6cm}|m{3.0cm}|m{0.6cm}|}
\hline
\textbf{Dataset} & \textbf{SL$\rightarrow$TL} & \textbf{SC (\%)} & \textbf{p-value (SC vs NL)} & \textbf{c/b} & \textbf{p-value (SC vs NL+SC)} & \textbf{c/b} & \textbf{p-value (SC vs NL $\cup$ (NL+SC))} & \textbf{c/b} & \textbf{p-value (SC vs SC $\cup$ NL $\cup$ (NL+SC))} & \textbf{c/b} \\
\hline
\multirow{8}{*}{\parbox{1.2cm}{\centering Avatar\\-\\Verified}} & Java$\rightarrow$C & 96.7 & \cellcolor{red!40}{0.05} & 4/13 & 0.06 & 5/0 & 0.06 & 5/0 & 0.06 & 5/0 \\
 & Java$\rightarrow$C++ & 98.8 & 1.00 & 1/2 & 1.00 & 1/2 & 1.00 & 1/0 & 1.00 & 1/0 \\
 & Java$\rightarrow$Go & 92.9 & 0.82 & 11/9 & 0.09 & 10/3 & \cellcolor{green!40}{$<0.01$} & 12/1 & \cellcolor{green!40}{$<0.01$} & 12/0 \\
 & Java$\rightarrow$Python & 97.1 & \cellcolor{red!40}{0.03} & 5/16 & 0.75 & 4/6 & 0.45 & 5/2 & 0.06 & 5/0 \\
 & Python$\rightarrow$C & 89.5 & 0.81 & 8/10 & 0.82 & 11/9 & \cellcolor{green!40}{0.04} & 12/3 & \cellcolor{green!40}{$<0.01$} & 12/0 \\
 & Python$\rightarrow$C++ & 95.8 & 0.23 & 3/8 & 0.38 & 1/4 & 1.00 & 3/3 & 0.25 & 3/0 \\
 & Python$\rightarrow$Go & 88.3 & 0.10 & 13/24 & 0.86 & 16/14 & \cellcolor{green!40}{0.02} & 18/6 & \cellcolor{green!40}{$<0.01$} & 18/0 \\
 & Python$\rightarrow$Java & 97.9 & 1.00 & 4/3 & 0.69 & 4/2 & 0.12 & 4/0 & 0.12 & 4/0 \\
\hline
\multirow{19}{*}{Codenet} & C$\rightarrow$C++ & 97.5 & 0.62 & 3/1 & 0.12 & 4/0 & 0.12 & 4/0 & 0.12 & 4/0 \\
 & C$\rightarrow$Go & 95.5 & 0.51 & 6/3 & \cellcolor{green!40}{0.03} & 6/0 & \cellcolor{green!40}{0.02} & 7/0 & \cellcolor{green!40}{0.02} & 7/0 \\
 & C$\rightarrow$Java & 98.5 & \cellcolor{red!40}{0.04} & 1/8 & 1.00 & 2/1 & 1.00 & 2/1 & 0.50 & 2/0 \\
 & C$\rightarrow$Python & 97.0 & \cellcolor{red!40}{0.01} & 2/12 & \cellcolor{red!40}{$<0.01$} & 1/13 & 1.00 & 3/3 & 0.25 & 3/0 \\
 & C++$\rightarrow$C & 99.5 & 0.22 & 1/5 & 0.22 & 1/5 & 0.62 & 1/3 & 1.00 & 1/0 \\
 & C++$\rightarrow$Java & 99.5 & 0.07 & 1/7 & 1.00 & 1/0 & 1.00 & 1/0 & 1.00 & 1/0 \\
 & C++$\rightarrow$Python & 95.5 & \cellcolor{red!40}{0.03} & 5/16 & 0.12 & 4/11 & 0.34 & 7/3 & \cellcolor{green!40}{0.02} & 7/0 \\
 & Go$\rightarrow$C & 96.5 & 0.23 & 3/8 & 1.00 & 5/4 & 0.22 & 5/1 & 0.06 & 5/0 \\
 & Go$\rightarrow$C++ & 98.5 & 0.29 & 2/6 & 1.00 & 2/3 & 1.00 & 2/1 & 0.50 & 2/0 \\
 & Go$\rightarrow$Java & 100.0 & 0.06 & 0/5 & 0.25 & 0/3 & 1.00 & 0/1 & 1.00 & 0/0 \\
 & Go$\rightarrow$Python & 94.0 & 0.08 & 4/12 & 0.45 & 6/10 & 1.00 & 6/5 & \cellcolor{green!40}{0.03} & 6/0 \\
 & Java$\rightarrow$C & 97.5 & 1.00 & 4/4 & 0.62 & 3/1 & 0.12 & 4/0 & 0.12 & 4/0 \\
 & Java$\rightarrow$C++ & 98.0 & 0.06 & 0/5 & 0.62 & 1/3 & 1.00 & 1/1 & 1.00 & 1/0 \\
 & Java$\rightarrow$Go & 93.5 & 1.00 & 6/6 & 1.00 & 6/6 & 0.07 & 9/2 & \cellcolor{green!40}{$<0.01$} & 9/0 \\
 & Java$\rightarrow$Python & 95.5 & \cellcolor{red!40}{$<0.01$} & 3/16 & \cellcolor{red!40}{0.02} & 2/11 & 0.51 & 3/6 & 0.25 & 3/0 \\
 & Python$\rightarrow$C & 98.0 & 1.00 & 3/3 & 1.00 & 2/1 & 0.62 & 3/1 & 0.25 & 3/0 \\
 & Python$\rightarrow$C++ & 99.5 & 0.50 & 0/2 & 1.00 & 0/0 & 1.00 & 0/0 & 1.00 & 0/0 \\
 & Python$\rightarrow$Go & 97.5 & 0.11 & 2/8 & 1.00 & 1/1 & 0.50 & 2/0 & 0.50 & 2/0 \\
 & Python$\rightarrow$Java & 99.0 & 1.00 & 1/1 & 1.00 & 1/0 & 1.00 & 1/0 & 1.00 & 1/0 \\
\hline
\multirow{1}{*}{Evalplus} & Python$\rightarrow$Java & 81.1 & 0.73 & 5/3 & 0.45 & 5/2 & 0.07 & 7/1 & \cellcolor{green!40}{0.02} & 7/0 \\
\hline
\end{tabular}
}
\label{tab:significance_result}
\end{table*}

==> sonar_table.tex <==
\begin{table*}
\centering
\tiny
% \fontsize{7}{9}\selectfont % Sets font to 7pt with 8pt line spacing
\caption{Comparison of Critical and Blocker Issues (with the ratio of issues per 1000 NCLOC) Before and After Fixing in Translated Code: Using Source Code with \specS and \spec-Only. N: Using \specS. Only, N+S: Using Source and \specS.}

\begin{tabular}{|p{1.1cm}|p{.8cm}|p{.8cm}|p{1cm}|p{1cm}|p{1.3cm}|p{1cm}|p{1.2cm}|p{1.0cm}|}
\hline

\multirow{2}{*}{\textbf{Dataset}} & \textbf{Source} & \textbf{Target} & \multicolumn{2}{|c|}{\textbf{LIT~\citep{pan2024lost}}} & \multicolumn{2}{|c|}{\textbf{N}} & \multicolumn{2}{|c|}{\textbf{N+S}} \\ \cline{4-9}
 & \textbf{Lang.} & \textbf{Lang.} & \textbf{Before Fix} & \textbf{After Fix} & \textbf{Before Fix} & \textbf{After Fix} & \textbf{Before Fix} & \textbf{After Fix} \\ \hline
\multirow{8}{*}{\textbf{Avatar}} & Java & C & 338 (43.13) & 293 (39.72) & 286 (32.0) & 298 (33.34) & \colorbox{highlight}{269 (30.1)} & 272 (30.43) \\ 
 & Java & C++ & 97 (12.72) & 101 (13.54) & \colorbox{highlight}{96 (11.63)} & 97 (11.75) & 100 (12.11) & 98 (11.87) \\ 
 & Java & Go & \colorbox{highlight}{38 (4.66)} & \colorbox{highlight}{40 (4.66)} & 44 (4.96) & 44 (4.96) & 43 (4.85) & 45 (5.07) \\ 
 & Java & Python & 35 (7.56) & \colorbox{highlight}{27 (5.62)} & 36 (6.62) & 37 (6.81) & 32 (5.89) & 33 (6.07) \\ 
 & Python & C & 346 (46.13) & 294 (41.88) & 331 (37.55) & 344 (39.02) & \colorbox{highlight}{327 (37.09)} & 344 (39.02) \\ 
 & Python & C++ & 128 (18.95) & 116 (16.59) & \colorbox{highlight}{69 (8.64)} & 73 (9.14) & 77 (9.64) & 74 (9.27) \\ 
 & Python & Go & \colorbox{highlight}{21 (3.36)} & 34 (3.9) & 38 (4.31) & 39 (4.42) & 33 (3.74) & 42 (4.76) \\ 
 & Python & Java & 42 (7.24) & 53 (7.69) & \colorbox{highlight}{52 (6.74)} & 56 (7.26) & 53 (6.87) & 54 (7.0) \\ \hline
\multirow{20}{*}{\textbf{CodeNet}} & C & C++ & 281 (42.97) & 267 (41.84) & 332 (46.83) & 330 (46.55) & \colorbox{highlight}{296 (41.75)} & 298 (42.04) \\ 
 & C & Go & \colorbox{highlight}{22 (3.24)} & 22 (3.29) & 24 (3.72) & 24 (3.72) & 22 (3.41) & 23 (3.56) \\ 
 & C & Java & 38 (6.9) & 39 (6.64) & 42 (6.9) & 44 (7.23) & \colorbox{highlight}{34 (5.59)} & 38 (6.25) \\ 
 & C & Python & 17 (4.03) & 20 (4.71) & 18 (3.8) & 23 (4.86) & \colorbox{highlight}{15 (3.17)} & 18 (3.8) \\ 
 & C++ & C & 208 (34.5) & 209 (34.93) & 211 (35.5) & 209 (35.16) & \colorbox{highlight}{201 (33.82)} & 203 (34.15) \\ 
 & C++ & Go & \colorbox{highlight}{21 (3.33)} & 22 (3.45) & 23 (3.86) & 24 (4.03) & 27 (4.54) & 27 (4.54) \\ 
 & C++ & Java & 38 (7.33) & 41 (7.32) & 49 (8.24) & 51 (8.58) & \colorbox{highlight}{37 (6.22)} & 44 (7.4) \\ 
 & C++ & Python & 13 (3.5) & \colorbox{highlight}{11 (2.95)} & 23 (6.27) & 23 (6.27) & 18 (4.91) & 19 (5.18) \\ 
 & Go & C & 262 (39.75) & 271 (41.02) & \colorbox{highlight}{262 (31.34)} & 273 (32.66) & 272 (32.54) & 286 (34.21) \\ 
 & Go & C++ & 70 (11.04) & 74 (11.75) & 79 (10.29) & 85 (11.07) & \colorbox{highlight}{72 (9.38)} & 81 (10.55) \\ 
 & Go & Java & 46 (6.91) & \colorbox{highlight}{47 (6.8)} & 60 (8.5) & 68 (9.63) & 57 (8.07) & 62 (8.78) \\ 
 & Go & Python & 23 (5.81) & 20 (4.96) & 27 (5.34) & 29 (5.73) & \colorbox{highlight}{17 (3.36)} & 19 (3.76) \\ 
 & Java & C & 238 (42.72) & 222 (40.12) & \colorbox{highlight}{219 (30.57)} & 235 (32.8) & 239 (33.36) & 250 (34.9) \\ 
 & Java & C++ & 104 (17.39) & 104 (17.76) & 100 (13.0) & 99 (12.87) & \colorbox{highlight}{93 (12.09)} & 96 (12.48) \\ 
 & Java & Go & 17 (2.38) & 17 (2.49) & 20 (2.54) & 21 (2.67) & \colorbox{highlight}{15 (1.91)} & 17 (2.16) \\ 
 & Java & Python & 15 (4.32) & 14 (4.03) & 26 (5.1) & 27 (5.3) & \colorbox{highlight}{20 (3.92)} & \colorbox{highlight}{20 (3.92)} \\ 
 & Python & C & 263 (54.04) & 245 (48.97) & \colorbox{highlight}{235 (42.18)} & 237 (42.53) & 246 (44.15) & 248 (44.51) \\ 
 & Python & C++ & 36 (8.16) & 45 (10.2) & 35 (7.0) & \colorbox{highlight}{33 (6.6)} & 35 (7.0) & \colorbox{highlight}{33 (6.6)} \\ 
 & Python & Go & 14 (2.56) & \colorbox{highlight}{13 (2.37)} & 17 (3.01) & 17 (3.01) & 15 (2.66) & 15 (2.66) \\ 
 & Python & Java & 19 (4.5) & 22 (4.71) & \colorbox{highlight}{20 (4.09)} & 21 (4.3) & 22 (4.5) & 23 (4.7) \\ \hline
\textbf{EvalPlus} & Python & Java & 127 (55.24) & 140 (52.77) & \colorbox{highlight}{162 (47.68)} & 168 (49.44) & 165 (48.56) & 172 (50.62) \\ 
\hline
\end{tabular}
\label{tab:sonar_table}
\end{table*}

==> translation_gpt_result.tex <==
\begin{table*}
\centering
\footnotesize
\renewcommand{\arraystretch}{1.2} % Improve row spacing
\caption{\color{blue}Results using \specS only and \spec+code, in comparison with the baseline results~\mbox{\citep{pan2024lost}, using GPT-4}}
\resizebox{\textwidth}{!}{  
\begin{tabular}{|m{1.3cm}|m{1.2cm}|m{2.8cm}|m{1cm}|m{2.2cm}|m{2.2cm}|m{2.2cm}|}
\hline
\textbf{Dataset} & \textbf{Source Language} & \textbf{Target Languages(s)} & \textbf{Total Codes} & \textbf{Baseline Correctness} & \textbf{\specS only Correctness} & \textbf{\specS+Source Correctness} \\
\hline
\multirow{2}{*}{Avatar} & Java & C, C++, Go, Python & 960 & \textbf{75.21\%} & 57.08\% & 71.97\% \\ \cline{2-7}
 & Python & C, C++, Go, Java & 956 & 53.14\% & 50.62\% & \textbf{56.93\%} \\
\hline
\multirow{5}{*}{CodeNet} & C & C++, Go, Java, Python & \multirow{5}{*}{4000} & \textbf{83\%} & 62\% & 75.125\% \\ \cline{2-3} \cline{5-7}
 & C++ & C, Go, Java, Python &  & 80\% & 69.125\% & \textbf{81.625\%} \\ \cline{2-3} \cline{5-7}
 & Go & C, C++, Java, Python &  & \textbf{85.5\%} & 66.875\% & 79.25\% \\ \cline{2-3} \cline{5-7}
 & Java & C, C++, Go, Python &  & \textbf{81.3\%} & 60.75\% & 74\% \\ \cline{2-3} \cline{5-7}
 & Python & C, C++, Go, Java &  & 79.9\% & 74.5\% & \textbf{83\%} \\
\hline
Evalplus & Python & Java & 164 & 76.83\% & 77.44\% & \textbf{79.88\%} \\
\hline \hline
Total / Average (all) & - & - & 6080 & \textbf{76.86\%} & 64.8\% & 75.15\% \\
\hline
\end{tabular}
}
\label{tab:base_translation_result}
\end{table*}
